HRTF Estimation in the Wild

Head Related Transfer Functions (HRTFs) play a crucial role in creating immersive spatial audio experiences. However, HRTFs differ significantly from person to person, and traditional methods for estimating personalized HRTFs are expensive, time-consuming, and require specialized equipment. We imagine a world where your personalized HRTF can be determined by capturing data through earbuds in everyday environments. In this paper, we propose a novel approach for deriving personalized HRTFs that only relies on in-the-wild binaural recordings and head tracking data. By analyzing how sounds change as the user rotates their head through different environments with different noise sources, we can accurately estimate their personalized HRTF. Our results show that our predicted HRTFs closely match ground-truth HRTFs measured in an anechoic chamber. Furthermore, listening studies demonstrate that our personalized HRTFs significantly improve sound localization and reduce front-back confusion in virtual environments. Our approach offers an efficient and accessible method for deriving personalized HRTFs and has the potential to greatly improve spatial audio experiences.

==> sections/desriptions.tex <==
Figure 1. shows our system overview as a flow diagram. There are three panels. The left panel is labeled "Noise Sources" and shows a vector art of a washing machine, speaker, and sink. There are sound waves coming from these sources. The middle panel is labeled "In Ear Microphones and Head Movements". It shows a woman wearing earbuds with a washing machine in the backgorund and an arrow pointing to the earbuds. The third panel is labeled "Personalzied HRTF". It shows a 3D contour plot of an HRTF with DB Gain on the vertical axis plotted against frequency and elevation angle. 


Figure 2. shows a a system overview with more technical detail as a horizontal flow diagram. In the left panel is a picture of a woman sitting in a room with a loudspeaker present. The next panel shows an spectrogram visualization (Time vs Frequency) of the left and right ear binaural recording of the woman titled "Binaural recording of ambient music". There are subtle differences in the frequencies between the two ears and over time shown in the spectrograms. There is a neural network titled UNet that takes the two spectrograms as input and produces two outputs. These two outputs are heatmaps with time on the x axis and frequency on the y axis with the heatmap value labeled "Gain Factor". The heatmap shows frequencies which are boosted and cut. There is an arrow from these two heatmaps titled Head Tracking that shows two 3D contour plots of the left and right hrtf. They are plotted as Gain (dB) on the vertical axis plotted against frequency and elevation.


Figure 3. shows two pictures of a man zoomed in on the face/head. The first picture has facial tracking landmarks superimposed on the face to show our head tracking algorithm. The right picture is a closeup of the ear and shows the earbud used in the experiment. It is wired and goes firmly in the ear.


Figure 4. shows our training procedure as a horizontal flow diagram. The left panel is labeled "Original Sound Source" and shows a single spectrogram that is largely constant and contains mostly noise. The next panel is titled "Binaural Rendering" and shows two spectrograms that closely resemble the original sound source. However they show more frequency variation over time and between the ears. A Unet block connects the two binaural rendering spectrograms to two output heatmaps titled "Predicted Filtering" with time (x axis) frequency (y axis) and the heatmap value labeled Gain Factor. These heatmaps closely follow the frequency variations of the binaural rendering image, showing with frequencies are predicted as booste or cut. There is an arrow from these heatmas to two more heatmaps. The arrow is called "L1 Los" and the last heatmaps are called "Ground Truth Filtering" they are very similar to the predicted filtering heatmaps.

Figure 5. shows panels of line charts in a grid that is 4 wide and 2 high. The 4 panels horizontally are labeled phi = 0 degrees, phi = 10 degrees, phi = 20 degrees, phi = 30 degrees. In each panel the top graph is labeled left and the bottom is labeld right. All graphs have 2 lines plotted, one called Ground Truth and the other called Predicted. The y axis is Gain (dB) and the x axis is Frequency (Hz). In all 8 graphs, the ground truth and predicted lines go up and down but mostly stay very close to each other. The purpose of this graph is to show that the predicted values of the HRTF match the ground trouth values closely at both ears and 4 different elevation angles.

Table 1. shows 5 rows with 2 columns. The column titles are "Method" and "LSD (dB)". The values are Random RIEC Subject: 8.23, Generic HRTF: 7.32, Zandi et. al: 4.5, Ours: 4.38, Hu et al.: 3.5


Figure 6 is a bar chart with the y axis labeled Angular Error (deg) and the X axis showing different error metrics. The bar chart shows the error for 3 experiments across 3 different error metrics for a total of 9 bars grouped into 3 groups of 3. The legend shows the 3 methods as Generic, Ours, and Groud-Truth. The first error metric is titled "Total Angular Error" and the values are Generic: 22.8, Ours: 15.7, Groud-Truth: 13.6. The second is "Azimuth Error" and shows Generic: 13.2, Ours: 9.3, Groud-Truth: 8.6. The last one is "Elevation Error" and shows Generic: 16.2, Ours: 10.9, Groud-Truth: 9.3. All bars also have error bars, these are between 1-2 degrees on most bars.

Table 1. shows 3 rows with 2 columns. The column titles are "Method" and "Front-back confusion rate". The values are Generic: 29 percent plus or minus 5.4, Ours: 14.8 percent plus or minus 4.6, GT HRTF 9.6 percent plus or minus 4.2.
